Minimizing Energy Use of Mixed-Fleet Public Transit for Fixed-Route Service

Affordable public transit services are crucial for communities since they enable residents to access employment, education, and other services. Unfortunately, transit services that provide wide coverage tend to suffer from relatively low utilization, which results in high fuel usage per passenger per mile, leading to high operating costs and environmental impact. Electric vehicles (EVs) can reduce energy costs and environmental impact, but most public transit agencies have to employ them in combination with conventional, internal-combustion engine vehicles due to the high upfront costs of EVs. To make the best use of such a mixed fleet of vehicles, transit agencies need to optimize route assignments and charging schedules, which presents a challenging problem for large transit networks. We introduce a novel problem formulation to minimize fuel and electricity use by assigning vehicles to transit trips and scheduling them for charging, while serving an existing fixed-route transit schedule. We present an integer program for optimal assignment and scheduling, and we propose polynomial-time heuristic and meta-heuristic algorithms for larger networks. We evaluate our algorithms on the public transit service of Chattanooga, TN using operational data collected from transit vehicles. Our results show that the proposed algorithms are scalable and can reduce energy use and, hence, environmental impact and operational costs. For Chattanooga, the proposed algorithms can save $145,635 in energy costs and 576.7 metric tons of CO2 emission annually.

==> algo/cost_matrix.tex <==
\begin{algorithm}[!h]
 \caption{$\textbf{Cost}(\mathcal{V}, \mathcal{T}, \alpha_m)$}
 \label{algo:init_cost_matrix}


 $\calEC \leftarrow \textbf{zeros}(|\mathcal{V}|, |\mathcal{T}|)$


\For {$t \in \mathcal{T}$}
 {
    \For {$v \in \mathcal{V}$}
    {
    
     $\text{cost} \leftarrow \infty$

         $\text{time\_feasible}, \text{energy\_feasible} \leftarrow \textbf{Feasible}(\mathcal{A}, v, x)$

\If {$\text{time\_feasible} \land \text{energy\_feasible}$}
{
     

        $\text{cost} \leftarrow \textbf{EnergyCost}(\mathcal{A},v,t,\alpha_m)$
        
        
       $t_i \leftarrow \calT.index(t)$
       
       $v_i \leftarrow \calV.index(v)$

       }
      $\calEC[t_i][v_i] \leftarrow \text{cost}$
}

}
 \KwResult{$\calEC$}
\end{algorithm}



==> data/full/co2_emission/co2_emission.tex <==
\pgfplotstableread[col sep=comma,]{data/full/co2_emission/greedy_co2_full.csv}\greedyco
\pgfplotstableread[col sep=comma,]{data/full/co2_emission/real_co2_full.csv}\realco
\pgfplotstableread[col sep=comma,]{data/full/co2_emission/sim_anneal_co2_full.csv}\saco

\begin{revision}
\begin{figure}[h!]
\begin{tikzpicture}
\begin{axis}[
      boxplot/draw direction=y,
      xtick={1,2,3},
      xticklabels={{Real}, {Greedy}, {SA}},
      width=\columnwidth,
      height = 6cm,
      bugsResolvedStyle/.style={},
      ylabel={Daily CO$_{2}$ Emission [metric tons]},
      xlabel={Algorithms},
      ymin=25,
      ymax=40,
    ]
\addplot+[boxplot={box extend=0.25, draw position=1}, ColorReal, solid, fill=ColorReal!20, mark=x] table [col sep=comma, y=real] {\realco};
\addplot+[boxplot={box extend=0.25, draw position=2},ColorGreedy, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=greedy] {\greedyco};
\addplot+[boxplot={box extend=0.25, draw position=3}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=sim_anneal] {\saco};
\end{axis}
\end{tikzpicture}
\caption{CO$_2$ emissions for assignments using greedy algorithm (\textcolor{ColorLegendGreedy}{$\blacksquare$}) and simulated annealing (\textcolor{ColorLegendSimAnn}{$\blacksquare$})  for complete daily schedules,
compared to existing real-world assignments (\textcolor{ColorLegendReal}{$\blacksquare$}).}
	\label{fig:co2_full_sch}
\end{figure}
\end{revision}

==> data/full/co2_emission/perc/perc.tex <==
\pgfplotstableread[col sep=comma,]{data/full/co2_emission/perc/greedy_co2_perc.csv}\greedyco
\pgfplotstableread[col sep=comma,]{data/full/co2_emission/perc/sim_anneal_co2_perc.csv}\ipco

\begin{figure}
\begin{tikzpicture}
\begin{axis}[
      boxplot/draw direction=y,
      xtick={1,2,3},
      xticklabels={{Real}, {Greedy}, {SA}},
      width=\columnwidth,
      height = 6cm,
      bugsResolvedStyle/.style={},
         yticklabel=\pgfmathprintnumber{\tick}\,$\%$,
      ylabel={Percentage of CO$_2$ Emission reduced},
      xlabel={Algorithms},
      ymin=-4,
      ymax=5,
    ]
\addplot+[boxplot={box extend=0.25, draw position=2},ColorGreedy, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=greedy] {\greedyco};
\addplot+[boxplot={box extend=0.25, draw position=3}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=sim_anneal] {\ipco};
\end{axis}
\end{tikzpicture}
\caption{Percentage of CO$_2$ emissions reduced for assignments using greedy algorithm (\textcolor{ColorLegendGreedy}{$\blacksquare$}) and simulated annealing (\textcolor{ColorLegendSimAnn}{$\blacksquare$})  for complete daily schedules,
compared to existing real-world assignments }
	\label{fig:co2_full_sch_perc}
\end{figure}


==> data/full/costs/perc/perc.tex <==
\pgfplotstableread[col sep=comma,]{data/full/costs/perc/greedy_cost_perc.csv}\greedyco
\pgfplotstableread[col sep=comma,]{data/full/costs/perc/sim_anneal_cost_perc.csv}\ipco

\begin{figure}
\begin{tikzpicture}
\begin{axis}[
      boxplot/draw direction=y,
      xtick={1,2,3},
      xticklabels={{Real}, {Greedy}, {SA}},
      width=\columnwidth,
      height = 6cm,
      bugsResolvedStyle/.style={},
      ylabel={Percentage of Energy Cost Saved},
      yticklabel=\pgfmathprintnumber{\tick}\,$\%$,
      xlabel={Algorithms},
      ymin=-4,
      ymax=5,
    ]
\addplot+[boxplot={box extend=0.25, draw position=2},ColorGreedy, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=greedy] {\greedyco};
\addplot+[boxplot={box extend=0.25, draw position=3}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=sim_anneal] {\ipco};
\end{axis}
\end{tikzpicture}
\caption{Percentage of Energy Cost saved for assignments using greedy algorithm (\textcolor{ColorLegendGreedy}{$\blacksquare$}) and simulated annealing (\textcolor{ColorLegendSimAnn}{$\blacksquare$})  for complete daily schedules,
compared to existing real-world assignments.
}
	\label{fig:cost_full_sch_perc}
\end{figure}


==> data/small/costs/costs.tex <==
\pgfplotstableread[col sep=comma,]{data/small/costs/greedy_costs.csv}\greedycost
\pgfplotstableread[col sep=comma,]{data/small/costs/sim_anneal_costs.csv}\simannealcost
\pgfplotstableread[col sep=comma,]{data/small/costs/ip_costs.csv}\ipcost

\begin{figure}
\begin{tikzpicture}
\begin{axis}[
      boxplot/draw direction=y,
      xtick={1,2,3,4,5,6,7,8,9,10,11,12},
      width=\columnwidth,
      height = 6cm,
      bugsResolvedStyle/.style={},
      ylabel={Energy Cost [\$]},
      xlabel={Number of Bus Lines},
      ymin=0,
      ymax=1400,
      legend pos=north west,
      legend cell align={left},
    ]
    \addlegendimage{ColorLegendIP, only marks, mark=square*};
    \addlegendentry{\,Integer Program};
    \addlegendimage{ColorLegendSimAnn, only marks, mark=square*};
    \addlegendentry{\,Simulated Anneal.};
    \addlegendimage{ColorLegendGreedy, only marks, mark=square*}
    \addlegendentry{\,Greedy Algorithm};
    
    \addplot+[boxplot={box extend=0.25, draw position=1},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_1] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=2},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_2] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=3},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_3] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=4},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_4] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=5},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_5] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=6},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_6] {\greedycost};
    \addplot+[boxplot={box extend=0.25, draw position=7},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_7] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=8},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_8] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=9},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_9] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=10},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_10] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=11},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_11] {\greedycost};
\addplot+[boxplot={box extend=0.25, draw position=12},ColorGreedy, rshift, solid, fill=ColorGreedy!20, mark=x] table [col sep=comma, y=line_12] {\greedycost};

    \addplot+[boxplot={box extend=0.25, draw position=1}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_1] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=2}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_2] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=3}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_3] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=4}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_4] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=5}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_5] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=6}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_6] {\simannealcost};
    \addplot+[boxplot={box extend=0.25, draw position=7}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_7] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=8}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_8] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=9}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_9] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=10}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_10] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=11}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_11] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=12}, ColorSimAnn, solid, fill=ColorSimAnn!20, mark=x] table [col sep=comma, y=line_12] {\simannealcost};
\addplot+[boxplot={box extend=0.25, draw position=1}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_1] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=2}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_2] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=3}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_3] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=4}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_4] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=5}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_5] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=6}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_6] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=7}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_7] {\ipcost};
\addplot+[boxplot={box extend=0.25, draw position=8}, ColorIP, lshift, solid, fill=ColorIP!20, mark=x] table [col sep=comma, y=line_8] {\ipcost};
7.07 \end{axis}
\end{tikzpicture}
\caption{Energy costs for assignments using the integer program (\textcolor{ColorLegendIP}{$\blacksquare$}), simulated annealing (\textcolor{ColorLegendSimAnn}{$\blacksquare$}), and the greedy algorithm~(\textcolor{ColorLegendGreedy}{$\blacksquare$}).}
	\label{fig:cost_all}
\end{figure}


==> related.tex <==
\section{Related Work}
\label{sec:related}

\citeauthor{wang2018bcharge}~\shortcite{wang2018bcharge}, \citeauthor{tian2016real}~\shortcite{tian2016real}, \citeauthor{wang2017data}~\shortcite{wang2017data} collect GPS data, bus stop data, bus transaction data, traffic data, and electricity consumption data, and use them to generate simulated models for energy prediction and optimization in transit networks. \citeauthor{santos2016towards}~\shortcite{santos2016towards} assume fixed costs, emission, and consumption rates for different types of vehicles, and \citeauthor{paul2014operation}~\shortcite{paul2014operation} assume fixed energy costs per unit distance without considering spatial and temporal factors. Unlike the previous research efforts, we derive realistic energy estimates using our energy predictors based on vehicle locations, traffic, elevation, and~weather data. 

Various approaches have been applied in the domain of energy optimization for bus transit networks. \citeauthor{chao2013optimizing}~\shortcite{chao2013optimizing} implement a genetic algorithm-based approach to minimize charging costs and operational costs separately.
\citeauthor{yang2020multi}~\shortcite{yang2020multi} implement a genetic algorithm based approach to minimize the energy and schedule multiple types of buses. \citeauthor{sun2020optimizing}~\shortcite{sun2020optimizing} use hybrid genetic algorithm by combining genetic algorithm and simulated annealing approach to optimize multi-terminal bus services. \citeauthor{santos2016towards}~\shortcite{santos2016towards} implements a non-dominated sorting genetic algorithm to assign buses considering energy consumption, environmental impact and service quality.
\citeauthor{wang2020optimal}~\shortcite{wang2020optimal} use dynamic programming for the optimization of scheduling charging for electric buses ensuring long lifetime of battery. \citeauthor{zhou2020collaborative}~\shortcite{zhou2020collaborative} use simulated annealing  to reduce energy cost and environmental impact. In addition, \citeauthor{li2014transit}~\shortcite{li2014transit} uses branch-and-price approach to solve smaller problem instances and uses column generation based heuristics to solve larger instances of the vehicle scheduling problem, with the objective of reducing the energy cost. \citeauthor{santos2016towards}~\shortcite{santos2016towards}, \citeauthor{zhou2020collaborative}~\shortcite{zhou2020collaborative}  worked on optimizing energy consumption of transit agencies operating mixed-fleets of vehicles.

Some works propose solutions that reduce energy costs by changing bus schedules or routes (e.g., \citeauthor{hassold2014improving}~\shortcite{hassold2014improving}, \citeauthor{wang2018bcharge}~\shortcite{wang2018bcharge}) which can cause inconvenience to passengers, while \citeauthor{santos2016towards}~\shortcite{santos2016towards} schedule buses ensuring that service level is unchanged. Further, some research efforts focus on optimizing the charging cost, charging schedule, and charging modes. \citeauthor{nageshrao2017charging}~\shortcite{nageshrao2017charging} use integer programming to optimize the charging costs of electric buses in the transit network. \citeauthor{wang2018bcharge}~\shortcite{wang2018bcharge} use Markov decision process for scheduling electric buses to charging stations. \citeauthor{jefferies2020comprehensive}~\shortcite{jefferies2020comprehensive} compare different ways of charging electric buses using greedy algorithm to the reduce the total cost. \citeauthor{gao2018electric}~\shortcite{gao2018electric} use a genetic algorithm-based approach to improve charging optimization. \citeauthor{9160687}~\shortcite{9160687} compare different charging infrastructures using integer programming to reduces the total ownership cost. \citeauthor{picarelli2020model}~\shortcite{picarelli2020model} use an integer programming-based solution to study the trade-off between the delaying trips to make a quick charge and serve the trip using electric buses rather than using costlier traditional buses. \citeauthor{olsen2020study}~\shortcite{olsen2020study} use space-time network for scheduling electric buses for charging.

\citeauthor{kliewer2006time}~\shortcite{kliewer2006time}, \citeauthor{kliewer2008line}~\shortcite{kliewer2008line}, \citeauthor{li2019mixed}~\shortcite{li2019mixed} allow a bus to serve multiple lines instead of limiting it to a single line, which can reduce energy cost; we also implement a similar approach. \citeauthor{li2019mixed}~\shortcite{li2019mixed} group the trips as origin-destination pairs and assign to vehicles, which also reduces energy costs. \citeauthor{li2014transit}~\shortcite{li2014transit} calculates the distance of deadheading trips by mapping a stop to the nearest intersection using point-to-curve matching, then solve one-to-one shortest-path problems using Dijkstra's algorithm, based on the road geometry data obtained from NavTeq.

\citeauthor{jahic2019preemptive}~\shortcite{jahic2019preemptive} apply preemptive, quasi preemptive, and non-preemptive approaches to optimally utilize the maximum load and eventually reduce electricity costs in charging stations or garages. Since charging time occupies a reasonable portion of the routine, \citeauthor{chao2013optimizing}~\shortcite{chao2013optimizing} propose a battery replacement technique, which reduces the complexity of scheduling with respect to charging, but it is not feasible when the number of electric buses is small, since purchasing more battery would not be cost-effective. \citeauthor{murphey2012intelligent}~\shortcite{murphey2012intelligent} present the development of a machine learning framework for energy management optimization in an HEV, developing algorithms based on long and short term knowledge about the driving environment.

